Reinforcement Learning: Stochastic Approximation Algorithms for Markov Decision Processes

This article presents a short and concise description of stochastic approximation algorithms in reinforcement learning of Markov decision processes. The algorithms can also be used as a suboptimal method for partially observed Markov decision processes.

==> part4/algorithmpomdp.tex <==
%!TEX root = ../book.tex



\chapter{Summary of Algorithms for Solving POMDPs} \label{chp:summary}

%\section*{Summary of Algorithms for Solving POMDPs}

For convenience, we  summarize various algorithms for solving POMDPs that appear in Parts II, III and IV of the book.
The algorithms can be classified into:


\subsection*{1. Optimal Algorithms}
For finite horizon POMDPs,
optimal algorithms are based on exact value iteration (which are  computationally intractable apart from small dimensional examples).
These are described in  \index{POMDP algorithm! Incremental Pruning}
\index{POMDP algorithm! Monahan's algorithm}  \index{POMDP algorithm! Witness algorithm} 
 \secn  \ref{sec:pomdpexactalgorithms} and include the Incremental Pruning Algorithm, Monahan's Algorithm and  Witness Algorithm.
Code for running these algorithms is freely downloadable from \url{http://www.pomdp.org}

 For discounted cost  infinite horizon POMDPs with discount factor $\discount$, based on Theorem \ref{thm:vipomdpgeom},
 running value iteration for $\iterfinal$ iterations yields an accuracy $$|\optvalue_\iterfinal(\belief) - \optvalue(\belief)| \leq \frac{\discount^{\iterfinal+1}}{1-\discount} \max_{\state,\action} |\cost(\state,\action)|$$
  
\subsection*{2. Suboptimal algorithms based on value iteration} 

%These were described in Chapters \ref{sec:lovejoy} and \ref{sec:pointbased}.
Lovejoy's algorithm in \secn s \ref{sec:lovejoy} provably sandwiches the optimal value function between low complexity lower and upper bounds.  \index{POMDP algorithm! Lovejoy's algorithm}
Lovejoy's algorithms is easily implementable in Matlab and can be run in conjunction with the POMDP solvers in
\url{http://www.pomdp.org}  

Point-based value iteration algorithms outlined in \secn  \ref{sec:pointbased} include SARSOP. Details and code can be obtained from
\url{http://bigbird.comp.nus.edu.sg/pmwiki/farm/appl/}  \index{POMDP algorithm! SARSOP algorithm}

The belief compression algorithm is outlined in \secn \ref{sec:compress}.
The open loop feedback control algorithm is described in \secn  \ref{sec:olfc}. 

\secn  \ref{sec:nonlinearpomdpmotivation} gives similar algorithms for POMDPs that have costs which are nonlinear in the belief state.
Such POMDPs arise in controlled sensing where one wishes to penalize uncertainty of the estimates.

%Chapter \ref{chp:saimm} gives one step lookahead based myopic policies for jump Markov linear systems. These are combined with state
%estimation algorithms for jump Markov linear systems.  Examples include the Sensor Adaptive IMM  Algorithm.

\subsection*{3. Algorithms that exploit POMDP structural results}

\secn  \ref{sec:radarkf} gives structural results for a stopping time problem involving Kalman filters in radar scheduling.
The costs involved are the stochastic observability (mutual information) of the targets. The optimal policy is a monotone
function of the covariance matrices with respect to the positive definite ordering.

 Chapter \ref{ch:pomdpstop}   gives structural results for stopping time POMDPs. 
For a variety of examples, sufficient conditions are given for the optimal policy to have a monotone structure on the belief space.
In \secn  \ref{sec:linear}, this monotone structure is exploited to devise  gradient algorithms that estimate the optimal linear monotone policy.
Algorithm \ref{alg:spsalinear} uses the SPSA algorithm to estimate the optimal linear monotone policy.  \index{POMDP algorithm! SPSA algorithm} \index{SPSA algorithm}


For more general POMDPs,
 Chapter \ref{chp:myopicul} presents structural results that provably upper and lower bound the optimal policy for a POMDP under 
certain assumptions. In this case, the upper and lower bounds are judiciously chosen myopic policies that can be computed via linear
programming. The upper and lower bound myopic policies  that optimize the overlap with the optimal POMDP policy are obtained
using linear programming in Algorithm \ref {alg1udit}.
Naturally once the myopic policies are obtained, their implementation is trivial.

\subsection*{4. Heuristics based on MDP Solutions}
The aim here is to use the value function or policy on the underlying MDP, and then combine this with the belief state in
various heuristic ways.


\secn  \ref{pomdpq} gives a Q-learning for POMDPs that is based on computing the Q-factors of the underlying  MDP.
Given the belief state $\belief$, compute  the POMDP policy as
$$ \policy(\belief) =   \argmax_\action \sum_\state \belief(\state) Q(\state,\action). $$
This is called  the Q-MDP algorithm in \cite{Cas98}.  \index{POMDP algorithm! Q-MDP algorithm}
For the above Q-MDP algorithm,  if the underlying MDP has the structure of Chapter \ref{chp:monotonemdp} so that the value function (and hence Q-factors)
are monotone, then this can be exploited. Similarly, if using the structural results
of Chapter \ref{chp:monotonemdp}, if the Q-factors are submodular, this property can also be exploited as a linear
constraint as described in \secn  \ref{chp:pdq} and a primal-dual Q-learning algorithm can be used. \index{primal-dual algorithm! Q-learning}



A simpler heuristic 
is to choose the POMDP policy as
$$\policy(\belief) =  \optpolicy_{\text{MDP}}(\hat{\state}_k) $$
where  $\optpolicy_{\text{MDP}}$ is computed via Q-learning on the underlying MDP and the clean state estimate $\hat{\state}_k$ is computed via the stochastic approximation algorithm
described in Chapter \ref{chp:markovtracksa}. Then no knowledge of the underlying POMDP parameters are required. 
In particular, if by using the structural results in Chapter \ref{chp:monotonemdp} 
it is established that the underlying MDP has a threshold policy, then $\policy(\belief)$ has a simple implementation.


\subsection*{5.  Gradient based policy search}  \index{POMDP algorithm! gradient policy search}
Chapter \ref{chp:rl} presents gradient based policy search algorithms for constrained MDP and POMDPs.
For the POMDP case (\secn  \ref{sec:pspomdp}), the algorithm proposed is model free in the sense that the parameters of the POMDP are
not required to be known. Define the state as a sliding window $\Delta$
of past actions and observations:
$$\state_k = (\obs_k, \obs_{k-1},\action_{k-1}, \obs_{k-2},\action_{k-2}, \ldots, \obs_{k-\Delta}, \action_{k-\Delta})$$
where $\Delta$ is a positive integer chosen by the user.
The aim is to determine the  optimal parameterized policy $\policy$ that maps $\state_k$ to $\action_k$.
A stochastic gradient algorithm is used to achieve this. The algorithm requires a gradient estimator to estimate
the gradient of the POMDP cost with respect to the policy. Both the score function  and weak derivative algorithms  are discussed 
in \secn  \ref{sec:sfmdp}   and \secn \ref{sec:wdmdp}, respectively. The score function algorithm was used in \cite{BB02}. 
The weak derivative method has significantly smaller variance as demonstrated in \secn  \ref{sec:numericalwd}.

\subsection*{6. Discrete Stochastic Optimization based search}  \secn  \ref{sec:dopt}  discusses several stochastic search algorithms
for estimating the best policy from a finite set of possible policies. Algorithm \ref{alg:adaptive-search}, \ref{alg:RS}  and 
\ref{alg:UCB} are examples.

\subsection*{7. Benchmark Problems}  \index{POMDP algorithm! benchmark problems}  \index{benchmark problems for POMDPs}
In the computational POMDP community, there are now several benchmark POMDP problems motivated by applications such as path planning,
and human-robot interaction. The following table from \cite{SPK13} lists some benchmark POMDP problems.

\begin{table}[h]
\begin{tabular}{|l|c|c|c|c|c|c|} \hline
Domain &  $\statedim$ & $\actiondim$ &  $\obsdim$ & Transitions & Observations & Horizon \\
\hline
Hallway \cite{LCK95} & 92 & 5 & 17 & stochastic & stochastic & 29 \\
Tag \cite{PGS03}   & 870  & 5 & 30 & stochastic & deterministic & 30 \\
Rocksample \cite{SS04}  & 12545 & 13 & 2 & deterministic & stochastic & 33 \\
Navigation \cite{KHL08} & 2653 & 6 & 102 & deterministic & deterministic & 62 \\
%Tiger grid & 36 & 5 & 17 & stochastic & stochastic & 8 \\
Wumpus 7 \cite{APG09} & 1568 & 4 & 2 & deterministic & deterministic & 16 \\  \hline
\end{tabular}

\end{table}





==> part4/frontmatter.tex <==

%!TEX root = ../book.tex
\part[Stochastic Approximation  and Reinforcement Learning]{Stochastic Approximation  and Reinforcement Learning
  \\ \\ \\ \\
                 % \begin{center}
                     \setstretch{0.6}  \begin{minipage}[l]{\textwidth} { %\setstretch{0.5}
                      \textmd{\normalsize 
  Parts II and III of the book discussed  stochastic  dynamic programming for POMDPs.
  The aim was to determine the globally optimal policy.
  Part IV deals with stochastic gradient algorithms that converge to a local optimum.
Such gradient algorithms are computationally efficient unlike dynamic programming which can be intractable.
Furthermore, stochastic gradient algorithms form the basis for reinforcement learning - that is, they facilitate estimating the optimal policy
when one does not know the parameters of the MDP or POMDP. %\\
%The stochastic gradient algorithm itself  is trivial to describe. It reads:\\
% $  \model_{k+1} = \model_k - \stepsize_k \hat\nabla_\model \Cost_k(\model_k) .$ 
%where $\model_k$ is the solution estimate at time $k$ and $\stepsize_k$ is a step size.
\\
Chapter \ref{chp:simulation} discusses gradient estimation for Markov processes
via stochastic simulation. This forms the basis of gradient based
reinforcement learning.
\\
Chapter \ref{chp:rl} presents simulation based stochastic approximation  algorithms for estimating the optimal policy of MDPs when the transition probabilities are not known. These algorithms are also described in the context of  POMDPs. The Q-learning algorithm and 
gradient based reinforcement learning algorithms are presented. \\
Chapter \ref{chp:markovtracksa} gives a brief description of convergence analysis of stochastic approximation algorithms. Examples
given include recursive maximum likelihood estimation of HMM parameters,  the least mean squares algorithm for estimating the state of an HMM
(instead of a Bayesian HMM filter), discrete stochastic optimization algorithms, and mean field dynamics for approximating the dynamics of information
flow in social networks.
 \\ Unlike Parts I to  III, Part IV of the book is non-Bayesian (in the sense that Bayes' formula is not the main theme).
}}
                     \end{minipage}
                %  \end{center}
                 }


